Differential Tracking Across Topical Webpages of Indian News Media

Online user privacy and tracking have been extensively studied in recent years, especially due to privacy and personal data-related legislations in the EU and the USA, such as the General Data Protection Regulation, ePrivacy Regulation, and California Consumer Privacy Act. Research has revealed novel tracking and personal identifiable information leakage methods that first- and third-parties employ on websites around the world, as well as the intensity of tracking performed on such websites. However, for the sake of scaling to cover a large portion of the Web, most past studies focused on homepages of websites, and did not look deeper into the tracking practices on their topical subpages. The majority of studies focused on the Global North markets such as the EU and the USA. Large markets such as India, which covers 20% of the world population and has no explicit privacy laws, have not been studied in this regard. We aim to address these gaps and focus on the following research questions: Is tracking on topical subpages of Indian news websites different from their homepage? Do third-party trackers prefer to track specific topics? How does this preference compare to the similarity of content shown on these topical subpages? To answer these questions, we propose a novel method for automatic extraction and categorization of Indian news topical subpages based on the details in their URLs. We study the identified topical subpages and compare them with their homepages with respect to the intensity of cookie injection and third-party embeddedness and type. We find differential user tracking among subpages, and between subpages and homepages. We also find a preferential attachment of third-party trackers to specific topics. Also, embedded third-parties tend to track specific subpages simultaneously, revealing possible user profiling in action.

==> Topical Tracking in Indian News Subpages (ArXiv) (1)/old-content.tex <==
\begin{comment}

The framework for DiBETS constitutes of the six components. %as depicted in the Figure~\ref{fig:dibets}. 
Entire framework uses data in the form of train websites (the top 25 URLs or our 123-URL dataset ordered by FB followers) and test websites (rest websites in the 123 websites list). Train websites are used to determine certain filtering parameters and mainly build the Topical Dictionary, which can further be repeatedly applied to any number of test websites. So, the components that consume the data of train websites do involve manual interventions as described further in detail. But, they are used only one-time initially to build the model, after which, the model enters into a completely automated phase. 

% \begin{figure*}
% \centering
%   \includegraphics[width=\textwidth, height=8cm]{samples/figures/DiBETS.pdf}
%   \caption{The Framework for DiBETS (Dictionary-Based Extractor of Topical Sub-pages) consisting of 6 components: URL Extractor, Parameterizer, Dictionary Builder, Filterer, Topic and Word Priority Setter, and Classifier.}
%   \label{fig:dibets}
% \end{figure*}

\subsection{The URL Extractor}
The first component is the URL Extractor Component which extracts all the URLs present in the homepage of a website. For a given homepage URL, URL Extractor Component uses an automated crawling script to scrape the HTML source page of the homepage. From the HTML content, all the valid URLs embedded in the homepage are extracted using HTML tags with an “href” attribute. We then segregate these URLs into internal URLs and external URLs. Internal URLs are the ones that belong to the same domain as that of the homepage. Contrastingly, external URLs have a different domain than the homepages. From 123 Indian News Websites in our dataset, our script could extract the HTML Pages of 112 websites (25 train and 87 test websites). In total, 15540 Internal URLs and 2718 External URLs were extracted for 112 websites. The URLs associated with the topic “epaper” often exist as external URLs. For example, the e-paper URL of “The Hindu” is “https://epaper.thehindu.com/“. Since, we consider “epaper” as a topic, we include only such epaper links from the external URLs to internal URLs and discard all the remaining external URLs from our analysis. If an internal URL doesn't terminate with '/' character, then '/' is appended at the end of the URL so that all URLs are in the same format before using them to determine various parameters in the Parameterizer Component.

\subsection{The Parameterizer}
From the URL Extractor Component, all the internal URLs of the test websites (11147 URLs) are then passed to the Filterer Component. The internal URLs of the train websites (4418 URLs) are passed to the Dictionary Builder Component to build a topical dictionary and to the Parameterizer Component to determine certain parameters with which to filter the internal URLs in the Filterer Component. We observed that the internal URLs mainly consists of two types of URLs -- sub-page URLs and direct URLs to the articles shown on the homepage of a website. Sub-page URLs on any homepage may consist URLs of a particular topical section shown on the homepage or URLs of topical sub-sub-sections or further nested topical pages. Since for all the websites, our ultimate objective is to find a single URL that represents the primary or main sub-page for each topic we consider, it is important to filter-out the article URLs from the internal URLs. Hence fundamentally, Parameterizer determines value of certain parameters that helps to separate-out the article URLs from the sub-page URLs. 

We hypothesized through manual observation that sub-page URLs are always shorter in length and direct article URLs are much longer lengthed. To check our hypothesis, in Parameterizer, we plotted a Histogram of length of the internal URLs with a bucket size of one. Histogram showcased a bi-modal distribution. %as depicted in the Figure~\ref{fig:params1}. 
The left distribution represents the sub-page URLs and the right one represents the article URLs. The two distributions are separated at a value of URL length of 80. Hence, we choose the \textit{URL Length < 80} as the first filtering parameter.

% \begin{figure}
% \centering
%   \includegraphics[width=\columnwidth]{samples/figures/Total URL Length P1.pdf}
%   \caption{Histogram of the Total Lengths of All Internal (sub-page + article) URLs of Train Websites (Bucket Size = 1)}
%   \label{fig:params1}
% \end{figure}

Furthermore, we observed that if we split a URL by the character '/' (slash) into different parts, then sub-page URLs have parts which are short-lengthed and have fewer '-' (hyphen) characters than the URLs of articles. For example, the sub-page URL "https://economicti-mes.indiatimes.com/wealth/personal-finance-news/aadhaar-card/" when split by '/' gives the following parts -- "https:", "" (empty part), "economictimes.indiatimes.com" (domain part), "wealth", "personal-finance-news", "aadhaar-card", and "" (empty part). From these parts we do not consider the first 3 parts and the last part for analysis since they are normal for all the websites and do not contribute in determining whether a given URL might belong to a sub-page or an article. However, if the word  'epaper' is present in the domain part, then we consider the domain part as well. The longest URL part in this URL has a length of 21. Also, it can be seen that the count of '-' in any part of the above URL has a maximum value of 2. On the other hand, if we consider the URL parts of an article URL like "https://www.rvcj.com/how-being-multi-lingual-can-benefit-your-nursing-career/" then it has longer-lengthed parts like "how-being-multi-lingual-can-benefit-your-nursing-career" with a length of 56 and a higher '-' count of 8. 

To confirm our hypothesis based on the length of URL parts and the count of hyphens, in Parameterizer, we plotted a histogram of the Length of URL parts %(see Figure~\ref{fig:params2}) 
with a bucket size 5 and a histogram of the count of hyphens in all URL parts (see Figure~\ref{fig:params3}) with a bucket size of 1. These plots were plotted without applying Parameter 1 filter to observe their distributions and set other parameters. Both of these histograms gave a bi-modal distribution aiding in determination of 2 additional parameters -- \textit{URL Part Length < 30} and a \textit{Hyphen Count < 4} for all URL parts within the URL. We observed that the first parameter of \textit{URL Length < 80} was self-sufficient to eliminate most of the article URLs, but still we applied the additional 2 parameters after applying the first one so as to remove any left-out article URLs (like the example discussed above). Statistically, from the 4418 Internal URLs of train websites that are sent to the Parameterizer, 2284 URLs have \textit{URL Length < 80}. We observed the count of filtered URLs when the Parameters 2 and 3 were separately applied on 4418 URLs to be 2295 and 2299 respectively. %(whose distribution is represented in Figures~\ref{fig:params2}) and \ref{fig:params3}.
From the Parameter 1 filtered 2284 URLs, the number of URLs which contain all \textit{URL Parts with Length < 30} were 2237 and separately, from the same 2284 URLs, the number of URLs which contain all parts with \textit{Hyphen Count < 4} were 2244. Also, applying Parameter 3 to URLs filtered by Parameter 1 and 2, showed a reduction of just 12 URLs. So, we concluded that applying Parameter 2 already removed almost all the URLs that didn't satisfy Parameter 3 and that Parameters 2 and 3 are almost inclusive of one-another. Also, both these parameters are related to URL-parts and checking these conditions together is a strong indicative of URL being a sub-page rather than an article URL. Hence, we decided to club the Parameters 2 and 3 together, leaving 2225 URLs behind. These 2225 URLs are sent to Dictionary Builder to generate the topical dictionary. All the three parameters determined in the Parameterizer are sent to the Filterer to use them to filter 11147 Internal URLs of test websites. 

% \begin{figure}
%   \subfigure[]{\centering \label{fig:params2}\includegraphics[width=\columnwidth]{samples/figures/Length of URL Parts P2.pdf}} \\
%   \subfigure[]{\centering \label{fig:params3}\includegraphics[width=\columnwidth]{samples/figures/Hyphen Counts in URL Parts P3.pdf}}
%   \caption{(a) Histogram of the Lengths of URL parts in all the Internal URLs of Train Websites (Bucket Size = 5) (b) Histogram of the Hyphen counts within each URL part of all the Internal URLs of Train Websites (Bucket Size = 1) (a) and (b) are without applying \textit{URL Length < 80}}
%   \label{fig:params23}
% \end{figure}

\subsection{The Filterer}
In Filterer, all the input internal URLs of test websites are first filtered by applying the filter of \textit{URL length} and then applying together the filters of \textit{URL Part Length} and \textit{Hyphen Count}. By applying these three filters, Filterer removes all the internal article URLs and outputs the candidate sub-page URLs. Candidate sub-page URLs are called so because these sub-page URLs are candidates for determining the single appropriate main sub-page URLs for each topic. The number of URLs remaining after applying each filter of Parameters 1, 2, and 3 separately were observed to be 6135, 5649, and 5798 respectively. The number of candidate sub-page URLs obtained by applying the filter of Parameter 1 followed by the filters of Parameter 2 and 3 together are 5342 URLs. These are sent to the classifier to detect primary sub-pages for each topic.

\subsection{The Topical Dictionary Builder}
The fundamental component of DiBETS is the Topical Dictionary Builder, which outputs a Topical Dictionary. This Dictionary is built by the human intervention using the input internal URLs of train websites from the Extraction Component and acts as a base to predict the topic to which a given sub-page URL of a website belongs to. To build the Topical Dictionary, we identified 24 distinct topic categories\footnote{astronomy and horoscope, automobiles, business and economics, coronavirus, crime, epaper, education and career, entertainment, factcheck, health and food, lifestyle and travel, opinions, politics, privacy policy, religion, science and technology, sitemap, sports, women, state and city news, world news, national news, latest news, media gallery} by manual observation of all the different topics discussed on homepages of some randomly visited Indian News Websites from our dataset. Furthermore, we also seek consent of an expert with a journalism background to verify that these 24 topics cover all the main topic categories discussed by the most Indian News Websites. Apart from these 24 topics, if we come across a sub-page that may belong to some different topic then we assign it a separate category - “other”. Sub-page URLs that get classified under "other" are the ones that cannot be mapped to one of 24 topics and are unimportant to study. We also clubbed similar topics like “business”, “finance”, and “economy” as a single topic “business and economics” so that we can represent and analyse only those topics which actually are fundamentally different. Also, such kind of clubbing made comparison across the websites uniform. Since, some website might have 'business' as a topical section and another website might not have 'business' but may have 'finance and economics' as a topical section.

To develop the topical dictionary, we manually scrutinized the content of each input internal URL and mapped it to one of the 25 topics. If the mapping could not be figured-out from the content of the URL, then we observed the actual content of the web-page represented by the URL by visiting that page. Next, from the URL content, we identified one or more keywords that were suggestive of or directly related to the identified topic. For example, for a URL "https://www.timesnownews.com/business-economy/budget/" mapped to the topic "business and economics", we identified 'business', 'economy', and 'economics', 'business-economy', 'budget' as keywords which are related to the topic "business and economy". Here, we avoided identifying words with a length of 3 or less if such keywords might create ambiguities. For example, the word 'fun' can be related to the topic 'entertainment' but this word acts as a sub-string in the words like 'mutual-funds' which should actually relate it to the topic 'business and economics', but instead due to 'fun', it can be identified as 'entertainment'. Its noteworthy that our topical dictionary based approach is better than normal word-net based approach because of two reasons -- one, for a topic like 'entertainment' for instance, word-net would add too many related words which might also include too generic keywords resulting in detecting the actual topic wrongly. Second, we select highly specific as well as their related words that are pertaining to only the content of Indian News Website's page URLs, hence it will create a highly domain-specific dictionary which will generalise well for other Indian News Websites also. Even our dictionary consists of a mix of 'Hindi' and 'English' language words, thereby capturing the common lingual terms by the Indian News Websites. Figure%~\ref{fig:topical dictionary} 
represents the words mapped to the topic "religion" in our topical dictionary capturing various "Hindi" related terms also which are used by the Indian News Website's in their sub-page URLs.

% \begin{figure}
% \centering
%   \includegraphics[width=7cm,height=7cm]{samples/figures/Topical Dict Religion.pdf}
%   \caption{Topical Dictionary showing Keywords for Topic "Religion". Topic Priority for the Topic is (\textit{L}) and Word Priorities of Keywords for "Religion" are shown in black triangles from 1 to 5 (1 = Highest and 5 = Lowest)}
%   \label{fig:topical dictionary}
% \end{figure}

We also assigned a Boolean label determining whether a given sub-page URL of a website is a main sub-page of one of the 24 topics or not by visiting the actual website. Once this process of identifying the topic, its associated keywords and the Boolean label for the main topical sub-pages was completed for all the filtered input internal URLs of train websites, we obtained a Topical Dictionary with topics as keys and bag-of-words for that topic as values. This dictionary was verified by the two subject experts and was then output by the Dictionary Builder and sent to the Classifier Component. The main sub-pages for all the identified topics in the set of URLs for train websites (i.e., Boolean label = 'Yes') were sent to the OpenWPM crawler so that we can analyze the tracking across different primary topical pages later on.

\subsection{The Topic \& Word Priority Setter}
With the help of the same two subject experts, we also associate priorities to the 25 topics and to the keywords associated with each topic in the Priority Setter Component.% (see example in Fig~\ref{fig:topical dictionary}). 
These priorities are also sent to the classifier Component. Priorities guide the classifier to determine which topic from the 25 topics should be given more importance or should be associated with a given URL, if the keywords of two or more topics are present within that URL. For instance, the topic 'state and city news' is given higher priority than the topic 'national news'. This is done so that the URLs like 'https://timesofindia.indiatimes.com/india/chhattisgarh/' don't get classified under 'national news' due to 'india' but get classified under 'state and city news' due to 'chhatisgarh' (a state in India). Topic Priorities are assigned with alphabetical letters where 'z' represents the highest priority and 'a' represents the 'lowest' priority and intermediate alphabets represents the relative priorities.

Similarly, if there are two or more sub-page URLs that are associated to the same topic, then priority of keywords within each topic's bag-of-words helps the classifier to decide which of those two or more sub-page URLs could be the main sub-page URL. For example in topic "health and food", words like 'health' or 'health-and-fitness' are assigned higher priorities than the words like 'yoga' or 'diet'. Moreover, for topics like "media gallery", we assigned higher priority to 'video' pages than 'photo' pages, since logically 'videos' are more informative. So, a URL containing higher priority words of a topic is highly probable to be the main sub-page URL for that topic. Priorities to the keywords within each topic are assigned on a scale of 1 to 5 (1 being the highest and 5 being the lowest priority). For assigning the priorities, all the labelled URLs of Dictionary Builder were closely examined.

\subsection{The Classifier}
The Classifier Component inputs the topical dictionary, the priorities of topics and keywords and the candidate sub-page links for the test websites. for each Indian News Website, it outputs a single main sub-page URL for all the topics from the 24 topics whose presence in detected in that website. This component uses the Algorithm 1 to predict the main sub-page URLs for different topics in each website. Our model can also be used to simply study the presence of different topics across a set of websites. The factors that we consider in assigning a topic to a particular internal sub-page URL are as computed from Lines 14 to 21. Variable $fraction\_presence$ tells us that to what extent a particular word from our topical dictionary matches to a particular part of the URL. For example, the extent to which 'sing' matches to a URL part 'dressing-style' in some URL is given by $fraction\_presence$ ~ 0.29, wherein this URL should be given lesser importance as compared to another URL where 'sing' exists in the URL part 'singing' with a $fraction\_presence$ ~ 0.57.

% \begin{algorithm}[h]
% 	\caption{Dictionary-based Prediction of Primary Sub-page URLs of Websites for each Topic}
% 	\label{algo}
% 	\scriptsize
% 	\begin{algorithmic}[1]
	
% 		%\Function{computeTHF}{$S_{h}$} %\Comment{Where A - array}
% 		\smallskip
% 		\State{Input $topical\_dictionary$, $topic\_priority$ and $word\_priority$.}
% 		\smallskip
% 		\State{Let $test\_websites$ = list of test Indian News Websites}
% 		\smallskip
% 		\State{Let $internal\_test\_URLs$ = Internal URLs of Test websites input from the Filterer}
		
% 		\smallskip
% 		\For{each $url$ in $test\_websites$}
% 		\smallskip
% 		\State{$subpage\_URLs$ = $internal\_test\_URLs$ of the current $url$}
% 		\smallskip
% 		\State{Let $link\_to\_topic\_mapping$ = empty dictionary}
        
%         \smallskip
%         \For{each $link$ in $subpage\_URLs$}
%         \smallskip
%         \State{$url\_parts$ = Split $link$ into non-empty parts as described in the Parameterizer}
%         \smallskip
%         \State{Let $link\_tuples$ = empty list}
        
%         \smallskip
%         \For{each $topic$ in $topical\_dictionary$}
        
%         \smallskip
%         \For{each $topic\_word$ in $topical\_dictionary[topic]$}
        
%         \smallskip
%         \For{each $part$ in $url\_parts$}
        
%         \smallskip
%         \If{$topic\_word$ in $part$}
%         \smallskip
%         \State{$fraction\_presence$ = length($topic\_word$) / length($part$)}
%         \smallskip
%         \If{$topic\_word$ in word tokenization of $part$}
%         \smallskip
%         \State{$completeness\_of\_presence = 1$}
%         \smallskip
%         \Else
%         \smallskip
%         \State{$completeness\_of\_presence = 0$}
%         \smallskip
%         \EndIf
%         \smallskip
%         \State{Add tuple$(topic, topic\_priority[topic], fraction\_presence,$} 
%         \State{$completeness\_of\_presence, topic\_word)$ to the $link\_tuples$}
%         \smallskip
%         \EndIf
        
%         \smallskip
%         \EndFor
        
%         \smallskip
%         \EndFor
        
%         \smallskip
%         \EndFor
        
%         \smallskip
%         \State{$sorted\_tuples$ = sort($link\_tuples$) in DESC by ($fraction\_presence$,}
%         \smallskip
%         \State{$completeness\_of\_presence, topic\_priority$ of the matched topic)}
        
%         \smallskip
%         \If{$fraction\_presence$ is 1.0 in first 2 $sorted\_tuples$ \& first has $topic$="other"}
%         \State{$label$ = assign first topic label from $sorted\_tuples$ which is not "other"}
%         \smallskip
%         \Else
%         \smallskip
%         \State{$label$ = assign first topic label from $sorted\_tuples$}
%         \smallskip
%         \EndIf
        
%         \smallskip
%         \State{$matching\_word$ = $topic\_word$ from the tuple whose $topic$ is assigned to $label$}
%         \smallskip
%         \State{$link\_to\_topic\_mapping[link]$ = a tuple$(label$, $matching\_word)$}

%         \smallskip
% 		\EndFor
		
% 		\smallskip
% 		\State{Let $main\_subpage\_URLs$ = empty dictionary}
		
% 		\smallskip
% 		\For{each $topic$ in $topical\_dictionary$}
% 		\smallskip
% 		\State{$topic\_subpage\_URLs$ = list of all sub-page URLs in $link\_to\_topic\_mapping$}
% 		\State{where assigned $label$ = current $topic$}
% 		\smallskip
% 		\State{$topic\_subpage\_URLs$ = sort($topic\_subpage\_URLs$) in ASC by length(URL)}
% 		\smallskip
% 		\State{$shortest\_URLs$ = first 3 shortest links in $topic\_subpage\_URLs$}
% 		\smallskip
% 		\State{$sorted\_URLs$ = sort($shortest\_URLs$) in ASC by }
% 		\State{(length(URL), $word\_priority$ of matching word in} 
% 		\State{$link\_to\_topic\_mapping[URL])$}
% 		\smallskip
% 		\State{$main\_subpage\_URLs[topic]$ = first link in $sorted\_URLs$}
% 		\smallskip
% 		\EndFor
		
% 		\smallskip
% 		\State{save($main\_subpage\_URLs$ as $[url\_domain]\_main\_subpages.json$)}
		
% 		\smallskip
% 		\EndFor
% 	\end{algorithmic}
% \end{algorithm}

The second factor $completeness\_of\_presence$ will be useful in deciding which URL is more important when both the URLs have the same value of $fraction\_presence$ < 1.0. Say for example, words 'culture' and 'economy' have the same $fraction\_presence$ ~ 0.37 in URL part 'agriculture-economy'. However, word 'culture' is absent in the word-tokenization of URL part 'agriculture-economy' (which when word-tokenized gives two words -- 'agriculture' and 'economy) but word 'economy' is present in the tokenized word list of this URL part. Hence, topic represented by 'economy' (i.e., topic 'business and economics') will be given more importance over the topic represented by 'culture' (i.e., 'entertainment'). The tuples obtained (refer Lines 20-21) for each word detected in any URL part are sorted first by the $fraction\_presence$, then by the $completeness\_of\_presence$ and lastly by $topic\_priority$ of the topic whose word matches as done in Lines 26-27.

Through manual inspection of internal URLs for train websites in Parameterizer, we observed that the URLs which were labelled as the main topical sub-pages for different topics in a website were almost always shortest-lengthed and seldomly second shortest in length. Based on this observation, we first assigned one of the 24 topics to all the internal as described above. Then, we decided to choose the 3 shortest-lengthed URLs (refer Line 41) for each topic towards determining which out of those 3 would be the main sub-page URL for that topic. To find out the main sub-page URL from these 3, we sorted the 3 URLs for each topic in ascending order, first, on the basis of length of the URL and then on the basis of $word\_priority$ of the dictionary word due to which the current topic label was assigned to that URL. 

Finally, for all the test websites, DiBETS outputs a single main sub-page URL for each of the 24 topics if they exist. This output labelled URLs are sent to the OpenWPM System for crawling various types of related data. It is important to note that the initial train phase involves determining various parameters in Parameterizer and building the Dictionary (in Dictionary Builder) followed by Setting the Priorities for topics and words (in Priority Setter). These Components involved in the train phase use only a small set of the train websites and involves manual effort as explained previously. However, once Topical Dictionary, Topic and Word Priorities and Parameter values are set, the entire model of DiBETS enters into a completely automated test phase and no longer requires the manual components of Parameterizer, Dictionary Builder and Priority Setter. 

\subsection{Brief Analysis}
To analyse the topics of interests for left, right, and centrist websites from the list of 112 websites that we could crawl, we first removed the 19 websites whose political leaning was "Not Known". Then, we plot the percentage of 93 websites belonging to different leanings for each topic. %as shown in Figure~\ref{fig:leaningwisetopics}. 
It is inferred from the plot that Only either Right or Left leaning websites are interested in the Topic \textit{Religion}. Also, the Right websites are more interested in \textit{Religion} than the left ones -- a trend also seen which topics like \textit{factcheck}, \textit{astronomy and horoscope} and \textit{automobiles}. On the other hand, the topics like \textit{opinions}, \textit{crime}, and \textit{E-paper\footnote{E-paper (electronic paper), image version of print publication e.g. \url{epaper.timesgroup.com/TOI/TimesOfIndia/index.html?a=c}}} are more talked-about by left-leaning websites than the right ones.

% \begin{figure}
% \centering
%   \includegraphics[width=\columnwidth]{samples/figures/Varying focus on Topics across different Political Leanings for 93 Indian News Websites.pdf}
%   \caption{Percentage of 93 news websites with their party-leanings for each of the 24 topics. The horizontal lines represent the percentage of 93 websites.}
%   \label{fig:leaningwisetopics}
% \end{figure}

\end{comment}

==> old-content.tex <==
\begin{comment}

The framework for DiBETS constitutes of the six components. %as depicted in the Figure~\ref{fig:dibets}. 
Entire framework uses data in the form of train websites (the top 25 URLs or our 123-URL dataset ordered by FB followers) and test websites (rest websites in the 123 websites list). Train websites are used to determine certain filtering parameters and mainly build the Topical Dictionary, which can further be repeatedly applied to any number of test websites. So, the components that consume the data of train websites do involve manual interventions as described further in detail. But, they are used only one-time initially to build the model, after which, the model enters into a completely automated phase. 

% \begin{figure*}
% \centering
%   \includegraphics[width=\textwidth, height=8cm]{samples/figures/DiBETS.pdf}
%   \caption{The Framework for DiBETS (Dictionary-Based Extractor of Topical Sub-pages) consisting of 6 components: URL Extractor, Parameterizer, Dictionary Builder, Filterer, Topic and Word Priority Setter, and Classifier.}
%   \label{fig:dibets}
% \end{figure*}

\subsection{The URL Extractor}
The first component is the URL Extractor Component which extracts all the URLs present in the homepage of a website. For a given homepage URL, URL Extractor Component uses an automated crawling script to scrape the HTML source page of the homepage. From the HTML content, all the valid URLs embedded in the homepage are extracted using HTML tags with an “href” attribute. We then segregate these URLs into internal URLs and external URLs. Internal URLs are the ones that belong to the same domain as that of the homepage. Contrastingly, external URLs have a different domain than the homepages. From 123 Indian News Websites in our dataset, our script could extract the HTML Pages of 112 websites (25 train and 87 test websites). In total, 15540 Internal URLs and 2718 External URLs were extracted for 112 websites. The URLs associated with the topic “epaper” often exist as external URLs. For example, the e-paper URL of “The Hindu” is “https://epaper.thehindu.com/“. Since, we consider “epaper” as a topic, we include only such epaper links from the external URLs to internal URLs and discard all the remaining external URLs from our analysis. If an internal URL doesn't terminate with '/' character, then '/' is appended at the end of the URL so that all URLs are in the same format before using them to determine various parameters in the Parameterizer Component.

\subsection{The Parameterizer}
From the URL Extractor Component, all the internal URLs of the test websites (11147 URLs) are then passed to the Filterer Component. The internal URLs of the train websites (4418 URLs) are passed to the Dictionary Builder Component to build a topical dictionary and to the Parameterizer Component to determine certain parameters with which to filter the internal URLs in the Filterer Component. We observed that the internal URLs mainly consists of two types of URLs -- sub-page URLs and direct URLs to the articles shown on the homepage of a website. Sub-page URLs on any homepage may consist URLs of a particular topical section shown on the homepage or URLs of topical sub-sub-sections or further nested topical pages. Since for all the websites, our ultimate objective is to find a single URL that represents the primary or main sub-page for each topic we consider, it is important to filter-out the article URLs from the internal URLs. Hence fundamentally, Parameterizer determines value of certain parameters that helps to separate-out the article URLs from the sub-page URLs. 

We hypothesized through manual observation that sub-page URLs are always shorter in length and direct article URLs are much longer lengthed. To check our hypothesis, in Parameterizer, we plotted a Histogram of length of the internal URLs with a bucket size of one. Histogram showcased a bi-modal distribution. %as depicted in the Figure~\ref{fig:params1}. 
The left distribution represents the sub-page URLs and the right one represents the article URLs. The two distributions are separated at a value of URL length of 80. Hence, we choose the \textit{URL Length < 80} as the first filtering parameter.

% \begin{figure}
% \centering
%   \includegraphics[width=\columnwidth]{samples/figures/Total URL Length P1.pdf}
%   \caption{Histogram of the Total Lengths of All Internal (sub-page + article) URLs of Train Websites (Bucket Size = 1)}
%   \label{fig:params1}
% \end{figure}

Furthermore, we observed that if we split a URL by the character '/' (slash) into different parts, then sub-page URLs have parts which are short-lengthed and have fewer '-' (hyphen) characters than the URLs of articles. For example, the sub-page URL "https://economicti-mes.indiatimes.com/wealth/personal-finance-news/aadhaar-card/" when split by '/' gives the following parts -- "https:", "" (empty part), "economictimes.indiatimes.com" (domain part), "wealth", "personal-finance-news", "aadhaar-card", and "" (empty part). From these parts we do not consider the first 3 parts and the last part for analysis since they are normal for all the websites and do not contribute in determining whether a given URL might belong to a sub-page or an article. However, if the word  'epaper' is present in the domain part, then we consider the domain part as well. The longest URL part in this URL has a length of 21. Also, it can be seen that the count of '-' in any part of the above URL has a maximum value of 2. On the other hand, if we consider the URL parts of an article URL like "https://www.rvcj.com/how-being-multi-lingual-can-benefit-your-nursing-career/" then it has longer-lengthed parts like "how-being-multi-lingual-can-benefit-your-nursing-career" with a length of 56 and a higher '-' count of 8. 

To confirm our hypothesis based on the length of URL parts and the count of hyphens, in Parameterizer, we plotted a histogram of the Length of URL parts %(see Figure~\ref{fig:params2}) 
with a bucket size 5 and a histogram of the count of hyphens in all URL parts (see Figure~\ref{fig:params3}) with a bucket size of 1. These plots were plotted without applying Parameter 1 filter to observe their distributions and set other parameters. Both of these histograms gave a bi-modal distribution aiding in determination of 2 additional parameters -- \textit{URL Part Length < 30} and a \textit{Hyphen Count < 4} for all URL parts within the URL. We observed that the first parameter of \textit{URL Length < 80} was self-sufficient to eliminate most of the article URLs, but still we applied the additional 2 parameters after applying the first one so as to remove any left-out article URLs (like the example discussed above). Statistically, from the 4418 Internal URLs of train websites that are sent to the Parameterizer, 2284 URLs have \textit{URL Length < 80}. We observed the count of filtered URLs when the Parameters 2 and 3 were separately applied on 4418 URLs to be 2295 and 2299 respectively. %(whose distribution is represented in Figures~\ref{fig:params2}) and \ref{fig:params3}.
From the Parameter 1 filtered 2284 URLs, the number of URLs which contain all \textit{URL Parts with Length < 30} were 2237 and separately, from the same 2284 URLs, the number of URLs which contain all parts with \textit{Hyphen Count < 4} were 2244. Also, applying Parameter 3 to URLs filtered by Parameter 1 and 2, showed a reduction of just 12 URLs. So, we concluded that applying Parameter 2 already removed almost all the URLs that didn't satisfy Parameter 3 and that Parameters 2 and 3 are almost inclusive of one-another. Also, both these parameters are related to URL-parts and checking these conditions together is a strong indicative of URL being a sub-page rather than an article URL. Hence, we decided to club the Parameters 2 and 3 together, leaving 2225 URLs behind. These 2225 URLs are sent to Dictionary Builder to generate the topical dictionary. All the three parameters determined in the Parameterizer are sent to the Filterer to use them to filter 11147 Internal URLs of test websites. 

% \begin{figure}
%   \subfigure[]{\centering \label{fig:params2}\includegraphics[width=\columnwidth]{samples/figures/Length of URL Parts P2.pdf}} \\
%   \subfigure[]{\centering \label{fig:params3}\includegraphics[width=\columnwidth]{samples/figures/Hyphen Counts in URL Parts P3.pdf}}
%   \caption{(a) Histogram of the Lengths of URL parts in all the Internal URLs of Train Websites (Bucket Size = 5) (b) Histogram of the Hyphen counts within each URL part of all the Internal URLs of Train Websites (Bucket Size = 1) (a) and (b) are without applying \textit{URL Length < 80}}
%   \label{fig:params23}
% \end{figure}

\subsection{The Filterer}
In Filterer, all the input internal URLs of test websites are first filtered by applying the filter of \textit{URL length} and then applying together the filters of \textit{URL Part Length} and \textit{Hyphen Count}. By applying these three filters, Filterer removes all the internal article URLs and outputs the candidate sub-page URLs. Candidate sub-page URLs are called so because these sub-page URLs are candidates for determining the single appropriate main sub-page URLs for each topic. The number of URLs remaining after applying each filter of Parameters 1, 2, and 3 separately were observed to be 6135, 5649, and 5798 respectively. The number of candidate sub-page URLs obtained by applying the filter of Parameter 1 followed by the filters of Parameter 2 and 3 together are 5342 URLs. These are sent to the classifier to detect primary sub-pages for each topic.

\subsection{The Topical Dictionary Builder}
The fundamental component of DiBETS is the Topical Dictionary Builder, which outputs a Topical Dictionary. This Dictionary is built by the human intervention using the input internal URLs of train websites from the Extraction Component and acts as a base to predict the topic to which a given sub-page URL of a website belongs to. To build the Topical Dictionary, we identified 24 distinct topic categories\footnote{astronomy and horoscope, automobiles, business and economics, coronavirus, crime, epaper, education and career, entertainment, factcheck, health and food, lifestyle and travel, opinions, politics, privacy policy, religion, science and technology, sitemap, sports, women, state and city news, world news, national news, latest news, media gallery} by manual observation of all the different topics discussed on homepages of some randomly visited Indian News Websites from our dataset. Furthermore, we also seek consent of an expert with a journalism background to verify that these 24 topics cover all the main topic categories discussed by the most Indian News Websites. Apart from these 24 topics, if we come across a sub-page that may belong to some different topic then we assign it a separate category - “other”. Sub-page URLs that get classified under "other" are the ones that cannot be mapped to one of 24 topics and are unimportant to study. We also clubbed similar topics like “business”, “finance”, and “economy” as a single topic “business and economics” so that we can represent and analyse only those topics which actually are fundamentally different. Also, such kind of clubbing made comparison across the websites uniform. Since, some website might have 'business' as a topical section and another website might not have 'business' but may have 'finance and economics' as a topical section.

To develop the topical dictionary, we manually scrutinized the content of each input internal URL and mapped it to one of the 25 topics. If the mapping could not be figured-out from the content of the URL, then we observed the actual content of the web-page represented by the URL by visiting that page. Next, from the URL content, we identified one or more keywords that were suggestive of or directly related to the identified topic. For example, for a URL "https://www.timesnownews.com/business-economy/budget/" mapped to the topic "business and economics", we identified 'business', 'economy', and 'economics', 'business-economy', 'budget' as keywords which are related to the topic "business and economy". Here, we avoided identifying words with a length of 3 or less if such keywords might create ambiguities. For example, the word 'fun' can be related to the topic 'entertainment' but this word acts as a sub-string in the words like 'mutual-funds' which should actually relate it to the topic 'business and economics', but instead due to 'fun', it can be identified as 'entertainment'. Its noteworthy that our topical dictionary based approach is better than normal word-net based approach because of two reasons -- one, for a topic like 'entertainment' for instance, word-net would add too many related words which might also include too generic keywords resulting in detecting the actual topic wrongly. Second, we select highly specific as well as their related words that are pertaining to only the content of Indian News Website's page URLs, hence it will create a highly domain-specific dictionary which will generalise well for other Indian News Websites also. Even our dictionary consists of a mix of 'Hindi' and 'English' language words, thereby capturing the common lingual terms by the Indian News Websites. Figure%~\ref{fig:topical dictionary} 
represents the words mapped to the topic "religion" in our topical dictionary capturing various "Hindi" related terms also which are used by the Indian News Website's in their sub-page URLs.

% \begin{figure}
% \centering
%   \includegraphics[width=7cm,height=7cm]{samples/figures/Topical Dict Religion.pdf}
%   \caption{Topical Dictionary showing Keywords for Topic "Religion". Topic Priority for the Topic is (\textit{L}) and Word Priorities of Keywords for "Religion" are shown in black triangles from 1 to 5 (1 = Highest and 5 = Lowest)}
%   \label{fig:topical dictionary}
% \end{figure}

We also assigned a Boolean label determining whether a given sub-page URL of a website is a main sub-page of one of the 24 topics or not by visiting the actual website. Once this process of identifying the topic, its associated keywords and the Boolean label for the main topical sub-pages was completed for all the filtered input internal URLs of train websites, we obtained a Topical Dictionary with topics as keys and bag-of-words for that topic as values. This dictionary was verified by the two subject experts and was then output by the Dictionary Builder and sent to the Classifier Component. The main sub-pages for all the identified topics in the set of URLs for train websites (i.e., Boolean label = 'Yes') were sent to the OpenWPM crawler so that we can analyze the tracking across different primary topical pages later on.

\subsection{The Topic \& Word Priority Setter}
With the help of the same two subject experts, we also associate priorities to the 25 topics and to the keywords associated with each topic in the Priority Setter Component.% (see example in Fig~\ref{fig:topical dictionary}). 
These priorities are also sent to the classifier Component. Priorities guide the classifier to determine which topic from the 25 topics should be given more importance or should be associated with a given URL, if the keywords of two or more topics are present within that URL. For instance, the topic 'state and city news' is given higher priority than the topic 'national news'. This is done so that the URLs like 'https://timesofindia.indiatimes.com/india/chhattisgarh/' don't get classified under 'national news' due to 'india' but get classified under 'state and city news' due to 'chhatisgarh' (a state in India). Topic Priorities are assigned with alphabetical letters where 'z' represents the highest priority and 'a' represents the 'lowest' priority and intermediate alphabets represents the relative priorities.

Similarly, if there are two or more sub-page URLs that are associated to the same topic, then priority of keywords within each topic's bag-of-words helps the classifier to decide which of those two or more sub-page URLs could be the main sub-page URL. For example in topic "health and food", words like 'health' or 'health-and-fitness' are assigned higher priorities than the words like 'yoga' or 'diet'. Moreover, for topics like "media gallery", we assigned higher priority to 'video' pages than 'photo' pages, since logically 'videos' are more informative. So, a URL containing higher priority words of a topic is highly probable to be the main sub-page URL for that topic. Priorities to the keywords within each topic are assigned on a scale of 1 to 5 (1 being the highest and 5 being the lowest priority). For assigning the priorities, all the labelled URLs of Dictionary Builder were closely examined.

\subsection{The Classifier}
The Classifier Component inputs the topical dictionary, the priorities of topics and keywords and the candidate sub-page links for the test websites. for each Indian News Website, it outputs a single main sub-page URL for all the topics from the 24 topics whose presence in detected in that website. This component uses the Algorithm 1 to predict the main sub-page URLs for different topics in each website. Our model can also be used to simply study the presence of different topics across a set of websites. The factors that we consider in assigning a topic to a particular internal sub-page URL are as computed from Lines 14 to 21. Variable $fraction\_presence$ tells us that to what extent a particular word from our topical dictionary matches to a particular part of the URL. For example, the extent to which 'sing' matches to a URL part 'dressing-style' in some URL is given by $fraction\_presence$ ~ 0.29, wherein this URL should be given lesser importance as compared to another URL where 'sing' exists in the URL part 'singing' with a $fraction\_presence$ ~ 0.57.

% \begin{algorithm}[h]
% 	\caption{Dictionary-based Prediction of Primary Sub-page URLs of Websites for each Topic}
% 	\label{algo}
% 	\scriptsize
% 	\begin{algorithmic}[1]
	
% 		%\Function{computeTHF}{$S_{h}$} %\Comment{Where A - array}
% 		\smallskip
% 		\State{Input $topical\_dictionary$, $topic\_priority$ and $word\_priority$.}
% 		\smallskip
% 		\State{Let $test\_websites$ = list of test Indian News Websites}
% 		\smallskip
% 		\State{Let $internal\_test\_URLs$ = Internal URLs of Test websites input from the Filterer}
		
% 		\smallskip
% 		\For{each $url$ in $test\_websites$}
% 		\smallskip
% 		\State{$subpage\_URLs$ = $internal\_test\_URLs$ of the current $url$}
% 		\smallskip
% 		\State{Let $link\_to\_topic\_mapping$ = empty dictionary}
        
%         \smallskip
%         \For{each $link$ in $subpage\_URLs$}
%         \smallskip
%         \State{$url\_parts$ = Split $link$ into non-empty parts as described in the Parameterizer}
%         \smallskip
%         \State{Let $link\_tuples$ = empty list}
        
%         \smallskip
%         \For{each $topic$ in $topical\_dictionary$}
        
%         \smallskip
%         \For{each $topic\_word$ in $topical\_dictionary[topic]$}
        
%         \smallskip
%         \For{each $part$ in $url\_parts$}
        
%         \smallskip
%         \If{$topic\_word$ in $part$}
%         \smallskip
%         \State{$fraction\_presence$ = length($topic\_word$) / length($part$)}
%         \smallskip
%         \If{$topic\_word$ in word tokenization of $part$}
%         \smallskip
%         \State{$completeness\_of\_presence = 1$}
%         \smallskip
%         \Else
%         \smallskip
%         \State{$completeness\_of\_presence = 0$}
%         \smallskip
%         \EndIf
%         \smallskip
%         \State{Add tuple$(topic, topic\_priority[topic], fraction\_presence,$} 
%         \State{$completeness\_of\_presence, topic\_word)$ to the $link\_tuples$}
%         \smallskip
%         \EndIf
        
%         \smallskip
%         \EndFor
        
%         \smallskip
%         \EndFor
        
%         \smallskip
%         \EndFor
        
%         \smallskip
%         \State{$sorted\_tuples$ = sort($link\_tuples$) in DESC by ($fraction\_presence$,}
%         \smallskip
%         \State{$completeness\_of\_presence, topic\_priority$ of the matched topic)}
        
%         \smallskip
%         \If{$fraction\_presence$ is 1.0 in first 2 $sorted\_tuples$ \& first has $topic$="other"}
%         \State{$label$ = assign first topic label from $sorted\_tuples$ which is not "other"}
%         \smallskip
%         \Else
%         \smallskip
%         \State{$label$ = assign first topic label from $sorted\_tuples$}
%         \smallskip
%         \EndIf
        
%         \smallskip
%         \State{$matching\_word$ = $topic\_word$ from the tuple whose $topic$ is assigned to $label$}
%         \smallskip
%         \State{$link\_to\_topic\_mapping[link]$ = a tuple$(label$, $matching\_word)$}

%         \smallskip
% 		\EndFor
		
% 		\smallskip
% 		\State{Let $main\_subpage\_URLs$ = empty dictionary}
		
% 		\smallskip
% 		\For{each $topic$ in $topical\_dictionary$}
% 		\smallskip
% 		\State{$topic\_subpage\_URLs$ = list of all sub-page URLs in $link\_to\_topic\_mapping$}
% 		\State{where assigned $label$ = current $topic$}
% 		\smallskip
% 		\State{$topic\_subpage\_URLs$ = sort($topic\_subpage\_URLs$) in ASC by length(URL)}
% 		\smallskip
% 		\State{$shortest\_URLs$ = first 3 shortest links in $topic\_subpage\_URLs$}
% 		\smallskip
% 		\State{$sorted\_URLs$ = sort($shortest\_URLs$) in ASC by }
% 		\State{(length(URL), $word\_priority$ of matching word in} 
% 		\State{$link\_to\_topic\_mapping[URL])$}
% 		\smallskip
% 		\State{$main\_subpage\_URLs[topic]$ = first link in $sorted\_URLs$}
% 		\smallskip
% 		\EndFor
		
% 		\smallskip
% 		\State{save($main\_subpage\_URLs$ as $[url\_domain]\_main\_subpages.json$)}
		
% 		\smallskip
% 		\EndFor
% 	\end{algorithmic}
% \end{algorithm}

The second factor $completeness\_of\_presence$ will be useful in deciding which URL is more important when both the URLs have the same value of $fraction\_presence$ < 1.0. Say for example, words 'culture' and 'economy' have the same $fraction\_presence$ ~ 0.37 in URL part 'agriculture-economy'. However, word 'culture' is absent in the word-tokenization of URL part 'agriculture-economy' (which when word-tokenized gives two words -- 'agriculture' and 'economy) but word 'economy' is present in the tokenized word list of this URL part. Hence, topic represented by 'economy' (i.e., topic 'business and economics') will be given more importance over the topic represented by 'culture' (i.e., 'entertainment'). The tuples obtained (refer Lines 20-21) for each word detected in any URL part are sorted first by the $fraction\_presence$, then by the $completeness\_of\_presence$ and lastly by $topic\_priority$ of the topic whose word matches as done in Lines 26-27.

Through manual inspection of internal URLs for train websites in Parameterizer, we observed that the URLs which were labelled as the main topical sub-pages for different topics in a website were almost always shortest-lengthed and seldomly second shortest in length. Based on this observation, we first assigned one of the 24 topics to all the internal as described above. Then, we decided to choose the 3 shortest-lengthed URLs (refer Line 41) for each topic towards determining which out of those 3 would be the main sub-page URL for that topic. To find out the main sub-page URL from these 3, we sorted the 3 URLs for each topic in ascending order, first, on the basis of length of the URL and then on the basis of $word\_priority$ of the dictionary word due to which the current topic label was assigned to that URL. 

Finally, for all the test websites, DiBETS outputs a single main sub-page URL for each of the 24 topics if they exist. This output labelled URLs are sent to the OpenWPM System for crawling various types of related data. It is important to note that the initial train phase involves determining various parameters in Parameterizer and building the Dictionary (in Dictionary Builder) followed by Setting the Priorities for topics and words (in Priority Setter). These Components involved in the train phase use only a small set of the train websites and involves manual effort as explained previously. However, once Topical Dictionary, Topic and Word Priorities and Parameter values are set, the entire model of DiBETS enters into a completely automated test phase and no longer requires the manual components of Parameterizer, Dictionary Builder and Priority Setter. 

\subsection{Brief Analysis}
To analyse the topics of interests for left, right, and centrist websites from the list of 112 websites that we could crawl, we first removed the 19 websites whose political leaning was "Not Known". Then, we plot the percentage of 93 websites belonging to different leanings for each topic. %as shown in Figure~\ref{fig:leaningwisetopics}. 
It is inferred from the plot that Only either Right or Left leaning websites are interested in the Topic \textit{Religion}. Also, the Right websites are more interested in \textit{Religion} than the left ones -- a trend also seen which topics like \textit{factcheck}, \textit{astronomy and horoscope} and \textit{automobiles}. On the other hand, the topics like \textit{opinions}, \textit{crime}, and \textit{E-paper\footnote{E-paper (electronic paper), image version of print publication e.g. \url{epaper.timesgroup.com/TOI/TimesOfIndia/index.html?a=c}}} are more talked-about by left-leaning websites than the right ones.

% \begin{figure}
% \centering
%   \includegraphics[width=\columnwidth]{samples/figures/Varying focus on Topics across different Political Leanings for 93 Indian News Websites.pdf}
%   \caption{Percentage of 93 news websites with their party-leanings for each of the 24 topics. The horizontal lines represent the percentage of 93 websites.}
%   \label{fig:leaningwisetopics}
% \end{figure}

\end{comment}
